Dense Fixed-Wing Swarming using Receding-Horizon NMPC

In this paper, we present an approach for controlling a team of agile fixed-wing aerial vehicles in close proximity to one another. Our approach relies on receding-horizon nonlinear model predictive control (NMPC) to plan maneuvers across an expanded flight envelope to enable inter-agent collision avoidance. To facilitate robust collision avoidance and characterize the likelihood of inter-agent collisions, we compute a statistical bound on the probability of the system leaving a tube around the planned nominal trajectory. Finally, we propose a metric for evaluating highly dynamic swarms and use this metric to evaluate our approach. We successfully demonstrated our approach through both simulation and hardware experiments, and to our knowledge, this the first time close-quarters swarming has been achieved with physical aerobatic fixed-wing vehicles.

==> approach.tex <==
\section{Approach}

\subsection{Dynamics Model}

We extend the planar post-stall aircraft model presented in \cite{moore2014robust} into a three-dimensional model of a fixed-wing UAV. The extension of this model is first described in \cite{basescu2020icra} and an abbreviated version is revisited here.
We define our state as $\vect{x} = \begin{bmatrix} \vect{r}, \vectg{\theta}, \vectg{\delta}, \delta_t, \vect{v}, \vectg{\omega}\end{bmatrix}^T$. Here $\vect{r} =\begin{bmatrix} x_r,y_r,z_r\end{bmatrix}^T$ represents the position of the center of mass in the world frame $O_{x_r y_r z_r}$, $\vectg{\theta}= \begin{bmatrix} \phi, \theta, \psi\end{bmatrix}^T$ represents the set of $x-y-z$ Euler angles applied in a $ZYX$ intrinsic rotation sequence, and $\vectg{\delta} = \begin{bmatrix} \delta_{ar}, \delta_e, \delta_r \end{bmatrix}^T$ are control surface deflections for the right aileron, elevator, and rudder respectively. The left aileron deflection is treated as a dependent parameter, with $\delta_{al} = -\delta_{ar}$. $\delta_t$ is the magnitude of thrust from the propeller, $\vect{v} = \begin{bmatrix} v_x, v_y, v_z\end{bmatrix}^T$ is the velocity of the center of mass in the world frame, and $\vectg{\omega} = \begin{bmatrix}\omega_x, \omega_y, \omega_z\end{bmatrix}^T$ is the angular velocity of the body in the body-fixed frame $O_{xyz}$., and  $\vect{u}_{cs} = \begin{bmatrix} \omega_{ar}, \omega_{e}, \omega_{r}\end{bmatrix}^T$, where $\vect{u}_{cs}$ are the angular velocities of the control surfaces.
The equations of motion then become
\begin{align}
\dot{\vect{r}} &= \bR_b^r \vect{v},\quad \dot{\vectg{\theta}} = {\bT}_{\omega}^{-1}{\boldsymbol \omega}\nonumber\\
\dot{\vectg{\delta}} &= \vect{u}_{cs}, \quad \dot{\delta}_t = a_t \delta_t + b_t u_t\nonumber\\
\dot{\vect{v}} &= \vect{f}/m - \vectg{\omega}\times \vect{v},\quad \dot{\vectg{\omega}} = \matr{J}^{-1}(\vect{m}-\vectg{\omega}\times\matr{J}\vectg{\omega})
\label{eq:eom}
\end{align}

where 
\begin{align}
\vect{f}&= \sum_i\vect{f}_{s_i} - mg{\bR_b^r}^T \bez + {\bR_{t}^b}\vect{f}_{t} + \vect{f}_a\nonumber\\
\vect{m}&= \sum_{i}(\vect{l}_{s_i} \times \vect{f}_{s_i}) + \vect{m}_a .
\end{align}

Here $m$ is vehicle mass, $\matr{J}$ is the vehicle's inertia, $\bR_b^r$ denotes the rotation of the body-fixed frame with respect to the world frame, ${\bT}_{\omega}$ is the transformation which maps the Euler angle rates to an angular velocity in the body-fixed frame, $\bR_{t}^b$ is the rotation matrix that defines the orientation of the thrust source with respect to the body-fixed frame, and $g$ is the acceleration due to gravity. $\vect{f}_{s_i}$ represents the force due to each aerodynamic surface in the body frame calculated using flat plate theory and $\vect{f}_{t}$ represents the force due to the propeller and is given as $\vect{f}_{t}=\begin{bmatrix}\delta_{t} & 0 & 0\end{bmatrix}^T$. $\vect{l}_{s_i}$ is the vector from the vehicle center of mass to the surface center of pressure in the body-fixed frame. $a_t$ and $b_t$ are constants used to model the thrust dynamics and $u_t$ is the normalized control signal for the motor, $u_t\in{[0,1]} $. $\vect{f}_a$ and $\vect{m}_a$ represent learned residual aerodynamic forces and moments respectively.


\subsection{Trajectory Generation}

Direct trajectory optimization is characterized by the inclusion of both the inputs and states as decision variables in the optimization problem \cite{pardo2016evaluating} and often exhibits superior numerical conditioning and greater robustness to local minima than indirect methods \cite{tedrake2009underactuated}. Here, we use a direct transcription formulation of Simpson's integration rule as described in \cite{pardo2016evaluating} and formulate a trajectory optimization problem to solve the post-stall landing problem. We employ the Sparse Nonlinear Optimizer (SNOPT) \cite{Gill:2005:Snopt} to solve our nonlinear optimization problem. For the landing problem, even over fairly large ($\approx$ 4s) time horizons we have found that these implicit integration constraints offer good numerical stability and reduce the required number of knot points, which reduces the overall computational burden. Our trajectory optimization problem can be written as
\begin{equation}
\begin{aligned}
& \underset{\vect{x}_k, \vect{u}_k, h }{\text{min}}
& & \vect{\bar{x}}_N^T \vect{Q_f} \vect{\bar{x}}_N + \sum_k^{N-1}{ \vect{x}_k^T \vect{Q}  \vect{x}_k + \vect{u}_k^T \vect{R}  \vect{u}_k}\\
& \text{s.t.}
& & \vect{x}_{k} - \vect{x}_{k+1} + \frac{h}{6.0}(\vect{\dot{x}}_{k} + 4 \vect{\dot{x}}_{c,k} + \vect{\dot{x}}_{k+1})= 0\\
&
& & -\vectg{\delta}_f \le \vect{x}_{N}-\vect{x}_f \le \vectg{\delta}_f,~ -\vectg{\delta}_i \le \vect{x}_{0}-\vect{x}_i \le \vectg{\delta}_i\\
&
& & \vect{x}_{min}  \le \vect{x}_{k} \le \vect{x}_{max},~ \vect{u}_{min}  \le \vect{u}_{k} \le \vect{u}_{max}\\
&
&  & h_{min}  \le h \le h_{max},~ \forall k \in [0,\ldots,N]
\end{aligned}
\end{equation}
where 
\begin{align}
\vect{\dot{x}}_{k} &= \vect{f}(t, \vect{x}_{k}, \vect{u}_{k}),~~
\vect{\dot{x}}_{k+1} = \vect{f}(t, \vect{x}_{k+1}, \vect{u}_{k+1})\nonumber\\
\vect{u}_{c,k} &= (\vect{u}_{k} + \vect{u}_{k+1}) / 2\nonumber\\
\vect{x}_{c,k} &= (\vect{x}_{k} + \vect{x}_{k+1}) / 2 + h (\vect{\dot{x}}_{k} - \vect{\dot{x}}_{k+1}) / 8\nonumber\\
\vect{\dot{x}}_{c,k} &= \vect{f}(t, \vect{x}_{c,k}, \vect{u}_{c,k}).
\end{align}
Here, $\vect{x}$ is the system state and $\vect{u}$ is the control input. $h$ is the time step where $h_{min}=0.001s$ and $h_{max}=0.2s$. $\vectg{\delta}_f$ and $\vectg{\delta}_i$ represent the bounds on the desired final and initial states ($\vect{x}_f$,$\vect{x}_i$), respectively. $N$ is the number of knot points and $\bar{\vect{x}}_N = \vect{x}_N-\vect{x}_f$. $\matr{Q}$, $\matr{R}$, and $\matr{Q_f}$ are cost weighting matrices. In hardware, we achieved real-time planning at 5 Hz.
\subsubsection{Trajectory Tracking}
To control the aircraft to a trajectory between re-plans, we use time-varying LQR (TVLQR).
\begin{align}
\bu(t,\bx) &= \matr{K}(\bx-\bx_0(t))+\bu_{0}(t).
\end{align}
where the time-dependent feedback gain matrix $\matr{K}(t) = \matr{R_c}^{-1}\matr{B}(t)^T\matr{S}(t)$
and $\matr{S}(t)$ is computed by integrating
\begin{align}
-\dot{\matr{S}} = \matr{A}(t)^T\matr{S}+\matr{S}\matr{A}(t)-\matr{S}\matr{B}(t)\matr{R_c}^{-1}\matr{B}(t)^T\matr{S}+\matr{Q_c}
\end{align}
backwards in time from $t=T$ to $t=0$. Here $\matr{A}(t)=\frac{\partial \bff(\bx_0,\bu_0(t))}{\partial \bx}$ and $\matr{B}(t)=\frac{\partial \bff(\bx_0(t),\bu_0(t))}{\partial \bx}$. $\bx_{0}(t)$ and $\bu_{0}(t)$ are the nominal trajectories. $\matr{Q_c}$ and $\matr{R_c}$ are the weighting matrices on state and action respectively, and $\matr{S}(T)=\matr{Q_{fc}}$. Trajectory tracking occurred at a rate of 50 Hz. 

\subsection{Multi-Agent Architecture/Trajectory Passing}
\subsection{Statistical Verification}

==> background.tex <==
\section{background}

Background
\subsection{Swarm Energy Density}

==> discussion.tex <==
\section{Discussion}

Discussion
\subsection{Robust Selection of $\rho$}
Implementation of this planning algorithm for a particular robot swarm requires
tuning of the parameter $\rho$, the minimum allowable distance between agents.
The trajectory planner is constrained such that pairs of trajectories must be separated
by at least $\rho$.
The local controller must then be able to keep the agent within a tube of radius $\rho$ 
of the commanded trajectory.
$\rho$ should be selected by considering the performance of the tracking controller
- a controller that tracks trajectories tightly implies that agents can safely fly closer
together. 

We propose a method which quantifies the tracking performance for an agent with
stochastic dynamics, based on recorded trajectory data. From this data, one 
can construct a confidence bound on the probability of collision, resulting in a safe
choice of $\rho$.

The constraint of leaving the vicinity of the trajectory can be written as follows:
\begin{align}
    ||x(t), t|| < \rho
\end{align}

When the agent moves under stochastic dynamics, violations of this constraint can be represented
as a random variable $X$, whose value is 1 if the trajectory leaves the tube and 0 if it stays within.
Therefore,
\begin{align}
    P(||x(t), t|| \geq \rho) = \mathbb{E}[X]
\end{align}

From repeated samples of $X$, we wish to find a bound $\mathbb{E}[X]$ with an appropriate confidence level. 
To do this, we leverage Hoeffding's Inequality, which relates the difference between the sample mean and true 
expectation of a bounded random variable [CITATION].

\begin{align}
    P(|\bar{X} - \mathbb{E}[X]| > \gamma) \leq 2e^{-2N\gamma^{2}/(b-a)}
\end{align}

Where $\gamma$ is the difference between the sample and true means, $N$ is the number of samples, and $a, b$ 
are the lower and upper bounds of the random variable $X$. In our case, $X$ can take values of 0 or 1. Letting 
$\delta$ be the left hand side of the above inequality, we can rearrange to result in the following:

\begin{align}
    \mathbb{E}[X] \leq \bar{X} + \sqrt{\frac{-\ln(\delta /2)}{2N}}
\end{align}

$\delta$ can be interpreted to be the confidence in the bound. Given a desirable $\delta$, $\rho$ can
be selected such that the right hand side of the above inequality is sufficiently low, thus bounding the 
overall probability of constraint violation.

\subsection{Comparison of Various Maneuvers}

\subsection{Swarm Energy Density}
In order to characterize the performance of swarming robotic systems in complex maneuvers, we introduce a metric
which we call "Swarm Energy Density."
This metric can be used to score a swarming robotic system in terms of its speed, number of agents, and distance
between agents. 
The metric is given as follows:

\begin{align}
    \frac{\sum_i mv^{2}}{2V}
\end{align}

where $m$ is the mass of each agent, $v$ is the velocity of the agent, and $V$ is the volume of the smallest 
convex hull which fully envelops the swarm.

==> hardware.tex <==
\section{Experimental Results}

Hardware

==> introduction.tex <==
\section{Introduction}

Swarms of uncrewed aerial vehicles (UAVs) are able complete parallelizable tasks with greater speed and resilience than would be possible with a single robot. In particular, fixed-wing UAV swarms have the unique ability to leverage large lifting surfaces to achieve efficient flight and long range operations. However, to date, most UAV swarms have been comprised of multi-rotors, especially in cases where the UAVs must operate in close proximity to one another or other obstacles in the environment. By contrast, fixed-wing UAV swarms have often maintained large stand-off distances to avoid collisions. This is primarily due to the limited agility of fixed-wing UAVs. However, this limitation is not always due to the physical capabilities of the fixed-wing aircraft, but rather due to the inability of the underlying control algorithm to reason about the full flight envelope. In many instances, it would be advantageous to preserve both the long range capabilities of fixed-wing UAVs and the maneuverability of quadrotor UAVs.

In this paper, we present an approach for controlling multiple fixed-wing UAVs in close proximity to one another using receding-horizon nonlinear model predictive control (NMPC) so as to achieve both multi-rotor agility and fixed-wing range. Our approach relies on a direct transcription formulation of the trajectory optimization problem and is therefore able to encode both cost functions and constraints on the state variables. To prevent vehicle-vehicle collisions, we share trajectories among vehicles and leverage trajectory obstacle constraints. To ensure that vehicles stay close to their nominal trajectories, we employ a local time-varying feedback controller that is updated in real time, and characterize the performance of this feedback controller via statistical analysis to provide stochastic performance guarantees. 

We show that our approach is able to make use of a large portion of the flight envelope to enable close-quarters multi-vehicle operations. We demonstrate our approach in simulation with up to X agents, and demonstrate multiple multi-vehicle patterns in hardware, with up to four fixed-wing UAVs flying in close proximity. We also compare our results to other swarms in the literature in terms of a ``swarm energy density'' metric. To our knowledge, this is the first time dense fixed-wing swarming has been demonstrated in hardware. 


% \begin{figure}[]
%     \centering
%     \includegraphics[width=\columnwidth]{example-image-a}
%     \caption{Main image}
%     \label{fig:main_img}
% \end{figure}


==> related_work.tex <==
\section{Related Work}

Swarming with multi-rotors

Swarming with fixed-wing UAVs

NMPC for UAV control

With a few exceptions [e.g., (Hamer et al., 2018; Turpin et al., 2014)], approaches to swarm control
have been surprisingly limited in their ability to reason about the dynamics of individual agents.
Typically, swarm research has sought to develop coordinated behaviors for large numbers of agents
(Preiss et al., 2017) or to solve the multi-agent collision-free path planning problem (Arul et al.,
2019). However, this has often been done with extremely simplified dynamic or even kinematic
models (Chung et al., 2018). Even in the context of aerial swarm-on-swarm combat, agents have
maintained fairly conservative flight envelopes (McGrew et al., 2010; Strickland et al., 2018).


==> simulation.tex <==
\section{Simulation Results}

Simulation
